Security-Aware Approximate Spiking Neural Networks

Deep Neural Networks (DNNs) and Spiking Neural Networks (SNNs) are both known for their susceptibility to adversarial attacks. Therefore, researchers in the recent past have extensively studied the robustness and defense of DNNs and SNNs under adversarial attacks. Compared to accurate SNNs (AccSNN), approximate SNNs (AxSNNs) are known to be up to 4X more energy-efficient for ultra-low power applications. Unfortunately, the robustness of AxSNNs under adversarial attacks is yet unexplored. In this paper, we first extensively analyze the robustness of AxSNNs with different structural parameters and approximation levels under two gradient-based and two neuromorphic attacks. Then, we propose two novel defense methods, i.e., precision scaling and approximate quantization-aware filtering (AQF), for securing AxSNNs. We evaluated the effectiveness of these two defense methods using both static and neuromorphic datasets. Our results demonstrate that AxSNNs are more prone to adversarial attacks than AccSNNs, but precision scaling and AQF significantly improve the robustness of AxSNNs. For instance, a PGD attack on AxSNN results in a 72\% accuracy loss compared to AccSNN without any attack, whereas the same attack on the precision-scaled AxSNN leads to only a 17\% accuracy loss in the static MNIST dataset (4X robustness improvement). Similarly, a Sparse Attack on AxSNN leads to a 77\% accuracy loss when compared to AccSNN without any attack, whereas the same attack on an AxSNN with AQF leads to only a 2\% accuracy loss in the neuromorphic DVS128 Gesture dataset (38X robustness improvement).

==> Sections/Results-1.tex <==
\section{Results and Discussions}
\label{sec:results}
This section discusses the experimental setup and the impact of adversarial attacks and quantization on AxDNNs under adversarial settings (namely, adversarial approximation and adversarial quantization analysis) and tranferability of adversarial attacks from accurate DNNs to AxDNNs.
%==================================================================


\subsection{Experimental Setup}
In this paper, the accurate Lenet-5 (AccL5) and Alexnet (AccAlx) architectures are used with their baseline accuracy as 98\% and 81\%. The LeNet-5 architecture is comprised of two sets of convolutional and average pooling layers, followed by a flattening convolutional layer, two fully-connected layers and finally a softmax classifier. The Alexnet architecture contains five convolutional layers, three average pooling layers and two fully connected layers. 
For their approximate counterparts, the accurate multipliers in the convolutional layers are replaced with approximate unsigned multipliers using Evoapprox8b \cite{mrazek2017evoapproxsb} libraries. The approximate multipliers are employed in AxL5 and AxAlx according to their error resilience towards MNIST \cite{cohen2017emnist} and CIFAR-10 \cite{krizhevsky2009learning} classification e.g., those having accuracy less than 90\% and 75\% are discarded. The adversarial examples are generated using the Foolbox library \cite{rauber2017foolbox}. 


\subsection{Adversarial Approximation Analysis}
\label{subsec:advapprox}
To investigate the adversarial robustness of AxDNNs, this section discusses the impact of both gradient and decision-based attacks with reference to the first attack scenario in Section \ref{subsec:advknow}. 


\vspace{0.08in}
\subsubsection{\uline{Approximate DNNs under Gradient-Based Attacks}}

In AxDNNs, both approximation noise and adversarial robustness can be quantified in terms of mean average error (MAE) of the approximate multipliers. The lower the MAE is, the higher is the actual inference accuracy of AxDNNs (in the absence of adversarial attacks) and hence, higher is their adversarial robustness. For example, Fig. \ref{fig:LenetBIMFGM} shows that M8-based (MAE = 1.54\%) AxL5 exhibits 6\% inference accuracy lower than M7-based (MAE = 1.12\%) AxL5 in absence of any adversarial attack. Hence, it undergoes 11\% more accuracy loss under $\mathrm{\textit{l}}_\mathrm{\infty}$ norm-based BIM attack with $\epsilon$ = 0.2. It is also observed that two AxDNNs, having the same inference accuracy, behave in a similar fashion under the adversarial attacks. For instance, M2 and M3-based AxL5 perform close to AccL5 under the adversarial attacks due to their same inference accuracy. 

The adversarial robustness analysis in Fig. \ref{fig:LenetBIMFGM} also reveals that the accuracy and hence, adversarial robustness of AxDNNs decreases with an increase in the strength of the adversarial attack, even if the adversary is unaware of their inexact inference engine. For example, $\mathrm{\textit{l}}_\mathrm{\infty}$ norm-based BIM attack, with $\epsilon$ = 0.2, on AccL5 leads to 45\% decrease in accuracy. However, the same strength of the attack results into 75\% accuracy loss in M8-based AxL5 when compared to its accurate counterpart, where 8\% accuracy loss is contributed by approximate computing only (see Fig. 3(a)). Same trends are observed with other gradient-based attacks. 

It is also observed that AxDNNs, similar to accurate DNNs, exhibit more adversarial robustness under $\mathrm{\textit{l}}_\mathrm{2}$ norm-based attacks as compared to their $\mathrm{\textit{l}}_\mathrm{\infty}$ counterpart. This trend is noticeable with all adversarial attacks. For example, $\mathrm{\textit{l}}_\mathrm{\infty}$ norm-based FGM attack, with $\epsilon$ = 0.25, leads to 37\% accuracy loss in AccL5. The same attack leads to 45\% decrease in accuracy with M8-based AxL5 when compared to its accurate counterpart, where 5\% accuracy loss is contributed by approximate computing (see Fig. 3(c)). On the other hand, $\mathrm{\textit{l}}_\mathrm{2}$ norm-based FGM attack with $\epsilon$ = 0.25 causes almost no accuracy loss in both AccL5 and M9-based AxL5 (see Fig. 3(d)). The accuracy of M9-based AxL5 decreases initially with an increase in strength of such attack but then, increases around $\epsilon$ = 0.2 and drops again to 65\% with $\epsilon$ = 2. This small deviating defensive behavior is exceptional and very often observed in AxDNNs \textit{due to data-dependent discontinuity of their approximation-induced errors} \cite{guesmi2020defensive}. Such discontinuity can be referred to masking and non-masking of erroneous approximation bits which can traverse through the AxDNN layers.


Interestingly, Fig. \ref{fig:LenetBIMFGM}(d) shows a \uline{33\% accuracy loss in M9-based AxL5 but only 9\% accuracy loss in AccL5} is observed under $\mathrm{\textit{l}}_\mathrm{2}$ norm-based FGM attack with $\epsilon$ = 2. Likewise, Fig. \ref{fig:LenetPGDRAU} (a) shows a \uline{41\% accuracy loss in M9-based AxL5 but 17\% accuracy loss only in AccL5} is observed under the $\mathrm{\textit{l}}_\mathrm{2}$ norm-based PGD attack with $\epsilon$ = 2. Such trend is also observed with small perturbation budgets. For example, Fig. \ref{fig:LenetPGDRAU}(b) illustrate that $\mathrm{\textit{l}}_\mathrm{\infty}$ norm-based PGD attack with even $\epsilon$ = 0.05 leads to 28\% accuracy loss in M9-based AxL5 when compared to AccL5, which has only 1\% accuracy loss. This identifies non-defensive nature of AxDNNs under the adversarial attacks. This observation \textit{contradicts the defensive approximation} in \cite{guesmi2020defensive}, where approximate computing was rendered defensive with such adversarial attacks. Furthermore, the BIM (see Fig. 3(a) and Fig. 3(b)) and PGD attacks (see Fig. 4(a) and Fig. 4(b)) seem to have more impact on the adversarial robustness of both AccL5 and AxL5 in comparison to the FGM attacks. In case of AxAlx, the CIFAR-10 classification under adversarial attacks shows that their adversarial robustness is very close to AccAlx. Therefore, these results are excluded from the paper.   

\begin{figure}[!t]
\centering
	\begin{subfigure}[b]{.26\textwidth}
		\centering
		\vspace{-0.01in}
		\caption{$\mathrm{\textit{l}}_\mathrm{2}$-based CR Attack}
		{\resizebox{\textwidth}{!}{\input{Figs/l2CR.tikz}}\label{fig:l2CR}}
	\end{subfigure}
	\begin{subfigure}[b]{.21\textwidth}
		\centering
		\vspace{-0.01in}
		\caption{$\mathrm{\textit{l}}_\mathrm{2}$-based RAG Attack}
		{\resizebox{\textwidth}{!}{\input{Figs/l2RAG.tikz}}\label{fig:l2RAG}}
	\end{subfigure}
	\vspace{-0.02in}
	\caption{Adversarial robustness of accurate and approximate LeNet-5 under CR and RAG attacks with MNIST \cite{cohen2017emnist} dataset. The labels M1 to M9 refer to the 1JFF (Accurate), 96D, 12N4, 17KS, 1AGV, FTA, JQQ, L40 and JV3 multipliers in EvoApprox8b \cite{mrazek2017evoapproxsb} library.} 
	\label{fig:LenetCRRAG}
	\vspace{-0.23in}
\end{figure}


\subsubsection{\uline{Approximate DNNs under Decision-based Attacks}} 
%\vspace{-1mm}
The decision-based attacks affect the adversarial robustness of both AxDNNs and accurate DNNs. For example, Fig.\ref{fig:LenetPGDRAU}(d) shows that $\mathrm{\textit{l}}_\mathrm{\infty}$ norm-based RAU attack leads to 53\% accuracy loss in AccL5. However, the same attack leads to 80\% accuracy drop in M8-based AxL5, in comparison to its accurate counterpart, where 5\% accuracy loss is contributed by approximate computing only. Same trend in observed in case of other decision-based attacks. It is also noticed that the $\mathrm{\textit{l}}_\mathrm{2}$ norm-based decision-based attacks are comparatively less perturbing. However, their effect can be strong with an increase in the approximation noise in AxDNNs. Interestingly, $\mathrm{\textit{l}}_\mathrm{2}$-based CR attack in Fig. 5(a) undergoes \uline{almost zero percent accuracy loss in AccL5} inspite of high perturbation budget i.e., $\epsilon = 1.5$. However, the same attack has \uline{53\% accuracy drop with M8-based AxL5}, when compared to its accurate counterpart, where 5\% accuracy loss is contributed by approximate computing only (see Fig.\ref{fig:LenetCRRAG}). Furthermore, small deviations in these trends are observed in decision-based adversarial attacks as well but they do not cause significant changes in the accuracy. Similar adversarial robustness trend is observed with CIFAR-10 classification in case of decision-based attacks on Alexnet as shown in Fig. \ref{fig:alexnet}. It is also observed that AxAlx performs close to AccAlx and the impact of decision-based attacks is more noticeable in $\mathrm{\textit{l}}_\mathrm{\infty}$ norm-based RAU attack (see Fig. 6(d)).  

\subsection{Transferability Analysis} 
%\vspace{-1mm}
\label{subsec:transfer}
Adversarial examples are known for their transferability~\cite{adrel7}, which means that they are transferable from one model to another model. This also refers to the fact that it is possible to attack models to which the attacker does not have access~\cite{demontis2019adversarial}. Therefore, for further analyzing the adversarial robustness of AxDNNs, we craft the adversarial examples using accurate DNN models (second attack scenario discussed in Section \ref{subsec:advknow}) and evaluate their impact on AxDNNs with different model structures. Our results show that the adversarial attacks are more transferable if the adversary is not aware of both the inexactness and type of DNN model used in the inference engine. For example, Table \ref{tab:transfer} shows that $\mathrm{\textit{l}}_\mathrm{\infty}$ norm-based BIM attack ($\epsilon$ = 0.05), strongest attack in previous section, is more transferable from AccL5 to AxAlx, when compared to AxL5, and AccAlx to AxL5, when compared to AxAlx. Same trend is observed with both MNIST\cite{cohen2017emnist} and CIFAR-10 datasets. 

\begin{figure*}[!t]
\centering
	\begin{subfigure}[b]{.29\textwidth}
		\centering
		\vspace{-0.01in}
		\caption{$\mathrm{\textit{l}}_\mathrm{2}$-based CR Attack}
		{\resizebox{\textwidth}{!}{\input{Figs/l2CR_Alx.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
	\begin{subfigure}[b]{.23\textwidth}
		\centering
		\vspace{-0.01in}
		\caption{$\mathrm{\textit{l}}_\mathrm{2}$-based RAG Attack}
		{\resizebox{\textwidth}{!}{\input{Figs/l2RAG_Alx.tikz}}\label{fig:l2RAG_Alx}}
	\end{subfigure}
	\begin{subfigure}[b]{.23\textwidth}
		\centering
		\vspace{-0.01in}
		\caption{$\mathrm{\textit{l}}_\mathrm{2}$-based RAU Attack}
		{\resizebox{\textwidth}{!}{\input{Figs/l2RAU_Alx.tikz}}\label{fig:l2RAU_Alx}}
	\end{subfigure}
	\begin{subfigure}[b]{.23\textwidth}
		\centering
		\vspace{-0.01in}		\caption{$\mathrm{\textit{l}}_\mathrm{\infty}$-based RAU Attack}
		{\resizebox{\textwidth}{!}{\input{Figs/linfRAU_Alx.tikz}}\label{fig:linfRAU_Alx}}
	\end{subfigure}
	\vspace{-0.24in}
	\caption{Adversarial robustness of accurate and approximate Alexnet under CR, RAG and RAU attacks with CIFAR-10 \cite{krizhevsky2009learning} dataset. The labels M1 to M9 refer to the 1JFF (Accurate), 2P7, KEM, 150Q, 14VP, QJD, 1446 and GS2 multipliers in EvoApprox8b \cite{mrazek2017evoapproxsb} library.} 
	\label{fig:alexnet}
	\vspace{-0.15in}
\end{figure*}


\begin{figure}[!t]
	\centering
	\vspace{-0.05in}
	\includegraphics[width=1\linewidth]{Figs/Qacc2.pdf}
	%\vspace{-7mm}
	\caption{Adversarial robustness of quantized (qL5) and non-quantized accurate Lenet-5 (L5) under different adversarial attacks (with MNIST \cite{cohen2017emnist})}
	\label{fig:qAcc}
	\vspace{-0.2in}
\end{figure}

\begin{table}[!t]
\vspace{0.1in}
\caption {Transferability Analysis with $\mathrm{\textit{l}}_\mathrm{\infty}$ norm-based BIM Attack ($\epsilon$ = 0.05). X/Y represents accuracy before/after attack}
\vspace{0.1in}
\label{tab:transfer}
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\rowcolor[HTML]{E0E0E0} 
           & \multicolumn{2}{l|}{\cellcolor[HTML]{E0E0E0}MNIST} & \multicolumn{2}{l|}{\cellcolor[HTML]{E0E0E0}CIFAR-10} \\ \hline
\rowcolor[HTML]{E0E0E0} 
DNN Models & AxL5                     & AxAlx                   & AxL5                      & AxAlx                     \\ \hline&\\[-2ex]
AccL5      & 98/97                    & 67/43                   & 54/9                      & 53/4                      \\ \hline&\\[-2ex]
AccAlx     & 98/9                     & 67/11                   & 54/20                     & 53/10                     \\ \hline
\end{tabular}
\vspace{-0.1in}
\end{table}

\subsection{Adversarial Quantization and Approximation} 
\label{subsec:advquan}
Fig. \ref{fig:LenetBIMFGM} - Fig. \ref{fig:alexnet} present AxDNNs which employ approximate computing along-with quantization. From their comparison with 8-bit quantized accurate DNNs in Fig. \ref{fig:qAcc}, we observe that quantization improves the adversarial robustness \cite{khalid2019qusecnets}; however, approximate computing does not support this behavior. The classification accuracy of AxDNNs decreases with an increase in the strength of the adversarial attacks inspite of employing quantization. For example, under $\mathrm{\textit{l}}_\mathrm{\infty}$ norm-based PGD attack ($\epsilon$ = 0.2), the quantization increases the accuracy of non-quantized AccL5 by 58\% in Fig. \ref{fig:qAcc} (see label L5). Conversely, approximate computing decreases the accuracy of quantized AccL5 by 35\% in M8-based AxL5 under the same attack in Fig. \ref{fig:LenetPGDRAU}(b). The self-error inducing nature of approximate computing degrade the performance of quantized DNN models and hence, leads to successful adversarial attacks. Thus, the approximate computing acts antagonistic to quantization under the adversarial attacks. \\

\noindent \textit{Summary.} Most state-of-the-art AxDNNs employ approximate multipliers for reducing their energy consumption \cite{riaz2020caxcnn} \cite{marchisio2020red} \cite{spantidi2021positive}. These approximate multipliers either have approximate partial products generation or addition. However, approximation error in both cases depends on the \textit{specific} input bit combinations \cite{mazahir2019probabilistic}. Recently, Gusemi et al. exploited such approximation behavior in AxDNN for the defense against the fixed strength of the adversarial attacks \cite{guesmi2020defensive}. However, such defensive nature of AxDNNs is not always observable as shown by our experimental results in Section \ref{sec:results}. In a real-world scenario, the adversary can vary the perturbation budget which may lead to successful misclassification. For example, the input bits of approximate multipliers can have the input combinations, under different adversarial settings, for which their output has low approximation error in the same AxDNNs. Hence, the perturbed images may lead to successful adversarial attacks by rendering low approximation error in the output of approximate multipliers. Another interesting fact is that AxDNNs are not only vulnerable to higher perturbation budgets, but also to very small perturbations budgets in some cases, such as $\epsilon =0.05$ as shown in our experimental results. Note, an attack with such a small perturbations budget can be stealthy enough to bypass the attack detection techniques and remain imperceptible to human eye.

%We observed this phenomenon even for a very small perturbation budget ($\epsilon =0.05$) 

%\textbf{This is due to the fact (and shown in our experimental results), that the adversarial robustness of AxDNNs can vary under different adversarial settings with varying perturbation budgets.}





==> Sections/Sec4_MethodologyP.tex <==

\SetInd{0.5em}{0.5em}
\begin{algorithm}[!h]
	\caption{Precision Scaling for Robustness}
	\label{alg:robust}
        \small
		\footnotesize
        \DontPrintSemicolon

        \SetKwInOut{Input}{Inputs}\SetKwInOut{Output}{Outputs}
        \Input{Type of adversarial attack: $attack$ = PGD, BIM, Sparse Attack, Frame Attack etc. \\
        Time steps = $T$; \\
        Threshold Voltage = $V_{th}$; \\
        Train dataset: $\mathcal{D}_{tr}$ = ($X$, $L$); \\
        Test dataset: $\mathcal{D}_{ts}$ = ($x$, $l$); \\
        Perturbation budget = $\epsilon_i$, i = [1, p]; \\
        Precision level = $qt$ = 8 or 16 or 32 or around 0.01(DVS);\\
        Approximation threshold:$pt$; \\ 
        Quality constraint = $Q$ = accuracy\\
        Type of dataset $T_d$: 1 for neuromorphic else 0
        }

		\Output{Robustness level $R$ and scaled weights $w_q$}

		\begin{algorithmic}[1]
        \STATE ($model$, $w$) = accurateSNN ($V_{th}$, $T$, $\mathcal{D}_{tr}$)\\
        // Train SNN model  
        \IF {Accuracy ($model$) $\ge$ $Q$}{
            \STATE $adv$ = 0;
                \FOR {$k$ = 1 : size($\mathcal{D}_{ts}$)}{
                    \STATE ($x^{*}_k$, $l^{*}_k$) = AdvExGen ($model$, $\epsilon_i$, $attack$, $X^t_k$) \\ 
                    // Adversarial examples generation
                    \STATE $w'$ = AscendingOrder ($w$); \\
                    // Arrange weights in an ascending order
                    \STATE $Pi$ = min (1, $V_m^l$ / $V_{th}^l$); \\
                    // Find spike probability in each layer in every time step
                    \STATE $m_l^c$ = $\sum_{j=1}^{c} (w_j^c - qt)$; \\
                    // Mean of scaled weights for every connection $c$ in layer $l$
                    \STATE $w_q$ = (1/$N_s$) $T$ $m_l^c$ $C$ $P_i$ ; \\
                    // Weight scaling on the basis of $V_{th}$ and $T$
                    \STATE $w_q$ = Pruning ($w_q$, $pt$); \\
                    // Weight pruning
                    \STATE ($x'_k$, $l'_k$) = AdvAttacks ($model$, $\epsilon_i$, $attack$, $x^{*}_k$, $l^{*}_k$) \\ 
                    // Launch adversarial attack 
                    \IF{$T_d$ == 1}{
                       \STATE AQF($qt$,$model$, $\mathcal{D}_{ts}$) \\
                    //Apply Approximate Quantized Masked Filter for Neuromorphic Datasets
                    }\ENDIF
                    \IF {$l'_k$ $\neq$ $l_k$}{
                        \STATE adv++;}
                    \ELSE{
                        \STATE NOP;}
                    \ENDIF
                }\ENDFOR
                \STATE $R$ ($\epsilon_i$) = (1 - $adv$/ size($\mathcal{D}_{tr}$)) * 100; \\
                // Calculate robustness
                \IF {$R$ $\ge$ $Q$}{
                    \RETURN ($R$, $w_q$)
                }\ENDIF
         }\ENDIF 
        
\end{algorithmic}
\end{algorithm}




\section{precision-scaled AxSNN: Design Approach and Methodology}
\label{sec:methodology}

In this section, we discuss the key concepts behind robustifying AxSNNs through quantization and its corresponding design methodology in detail.

\subsection{Quantization for adversarial defense}

The approximation thresholds can be typically estimated by identifying the maximum tolerable perturbation (MTP) in a neural network \cite{khalid2019qusecnets}. However, this becomes challenging in precision-scaled AxSNNs due to their variation in accuracy with the change in the threshold voltage, time steps and quantization threshold which add another dimension to MTP exploration. To handle such problem, we determine approximation thresholds on the basis of the threshold voltage, time steps and quantization threshold. The threshold voltage  typically determines the probability of the spikes i.e., min $(1, V_m/ V_{th}$) which means that maximum spike probability is 1 when $V_m$ crosses $V_th$ otherwise, it is $V_m/ V_{th}$. Therefore, we utilize the probability of spikes to approximate and also, scale the weights. Specifically, we use the following equation: 

\begin{equation}
\label{eq:precision}
w_q = T / m c N_s \cdot min(1, V_m/V_{th})
\end{equation}


\noindent where the product $m c$ represents the significance of the spikes. Also $c$ and $m$ denote the number of connections to output and mean weight of the connections i.e., $\sum_{i=1}^{c} (w_i - p)$. Here, $p$ denotes the precision threshold (number of precision scales e.g., 2, 3, 4, ...). Higher the significance of the connections, less is the scaling of the weights. We assume that the spike probability is the same across all time steps. Specifically, find the scaled weights by averaging the inverse product of the probability of spikes and significance of the connections over the number of spikes $N_s$ in time steps $T$.   


\SetInd{0.5em}{0.5em}
\begin{algorithm}[!h]
	\caption{Approximate Quantized Filter:AQF}
	\label{alg:aqaf}
        \small
		\footnotesize
        \DontPrintSemicolon

        \SetKwInOut{Input}{Inputs}\SetKwInOut{Output}{Outputs}
        \Input{List of events:$(x,y,p,t) =E$\\
        Precision level = $qt$;\\
        }
		\Output{Filtered Quantized dataset $E$ and scaled weights $w_q$}
		\begin{algorithmic}[1]
        \STATE $M[128][128]=[0]$
        \STATE $activity=0$, $s=2$, $T1=5$ , $T2=30$
        \FOR {$e$ in E }{
        \STATE $e=round(e/qt)\cdot qt$
            \FOR {$i$ in $(x_e-s,x_e+s)$)}{
                 \FOR {$j$ in $(y_e-s,y_e+s)$ )}{
                    \IF{not($i==x_e$ and $j==y_e$)}{
                        \STATE $M[i][j] = t_e$
                    }\ENDIF
                    \IF{not($i==x_e$ and $j==y_e$)}{
                        \STATE $activity[i][j] += 1$
                    }\ENDIF
                }\ENDFOR
            }\ENDFOR
            \IF{$activity[i][j] > T1$}{
                        \STATE $M[i][j] = 1$
                }\ENDIF
            \IF{$t_e-M[x_e][y_e]>T2$ or $M[x_e][y_e]==1$)}{
               \STATE Remove $e$ from E
            }\ENDIF
        }\ENDFOR 
        
\end{algorithmic}
\end{algorithm}




\subsection{precision-scaled AxSNN Design Methodology}
In this section, we describe step-by-step how Equation \ref{eq:precision} can be used for precision scaling in AxSNN with reference to Algorithm 1. We first train a SNN model with the given set of threshold voltage $V_{th}$ and time steps $T$ and save the trained model and its corresponding weights (Line 1). This learning phase is quantitatively verified with a quality constraint $Q$ i.e., minimum baseline accuracy level below which we consider SNN learning inefficient (Line 2). The value of $Q$ depends on the given SNN architecture, its learning method, dataset and application. Next, we initialize a counter $adv$ for successful attack generation (Line 3). Then, we craft the adversarial examples for a given adversarial attack (Line 5). The adversarial defense through precision scaling starts from Line 6 where the trained weights are sorted initially in the ascending order. This sorting helps us in approximating the weights later. Afterwards, we determine the probability of spike generation in each layer in a time step (Line 7). The maximum probability of spike generation is 1 and the minimum is calculated by dividing the membrane potential $V_m$ with $V_{th}$. After this, we calculate the mean of all weights corresponding to a connection $c$ and use it for precision scaling of the weights (Line 8 and 9). We remove the connections having weights below approximation threshold (Line 10). In the case, of neuromorphic dataset our approximate quantization aware mask filter (AQF) as given in Algorithm \ref{alg:aqaf} is applied (Line 12) that removes perturbation noise for event-driven $e$ neuromorphic dataset $E$ in the form of $(x, y, p, t)$ the  x-coordinate, the y-coordinate, the polarity and the timestamp of the event e respectively. Next, the algorithm verifies if the crafted adversarial example is able to fool the approximate SNN  (Lines 14 -16), i.e., if the attack succeeded to force the output to a wrong label, and accordingly increment
the adversarial success counter. Lastly, we evaluate the robustness for $\epsilon$ as the rate of attacks for which the adversary failed to generate an adversarial example that fools the victim SNN (Lines 18 - 20). We use this algorithm to find the scaled weights for enhancing the robustness of the model.


\begin{figure}[!t]
	\centering
	%\vspace{-0.05in}
	\includegraphics[width=1\linewidth]{Figs/snngraph1.pdf}
	%\vspace{-7mm}
    \caption{Robustness analysis of approximate SNN MNIST classifier under PGD attack for different approximation levels.}
	\label{fig:approxlevel}
	\vspace{-0.15in}
\end{figure}

\begin{figure*}[!t]

\centering
	\begin{subfigure}[b]{.26\textwidth}
		\centering
		\vspace{-0.01in}		
        \caption{F32}
		{\resizebox{\textwidth}{!}{\input{Figs/q32pgd(2).tikz}}\label{fig:linfRAU_Alx}}
	\end{subfigure}
     \begin{subfigure}[b]{.22\textwidth}
    		\centering
    		\vspace{-0.01in}
    		\caption{F16}
    		{\resizebox{\textwidth}{!}{\input{Figs/q16pgdmnistep1(2).tikz}}\label{fig:l2RAU_Alx}}
    	\end{subfigure}
     \begin{subfigure}[b]{.22\textwidth}
		\centering
		\vspace{-0.01in}
        \caption{INT8}
		{\resizebox{\textwidth}{!}{\input{Figs/q8pgdmnistep1(2).tikz}}\label{fig:l2RAG_Alx}}
	\end{subfigure}
 \vspace{0.05in}

\centering
    \begin{subfigure}[b]{.262\textwidth}
    		\centering
    		\vspace{-0.01in}		
            %\caption{F32}
    		{\resizebox{\textwidth}{!}{\input{Figs/q32bim.tikz}}\label{fig:linfRAU_Alx}}
    	\end{subfigure}
	\begin{subfigure}[b]{.222\textwidth}
		\centering
		\vspace{-0.01in}		
        %\caption{F16}
		{\resizebox{\textwidth}{!}{\input{Figs/q16bimmnist.tikz}}\label{fig:linfRAU_Alx}}
	\end{subfigure}
	\begin{subfigure}[b]{.222\textwidth}
		\centering
		\vspace{-0.01in}		
        %\caption{INT8}
		{\resizebox{\textwidth}{!}{\input{Figs/q8bimmnist.tikz}}\label{fig:linfRAU_Alx}}
	\end{subfigure}
	\vspace{-0.24in} 

    \vspace{0.3in}
        \caption{Robustness of approximate and accurate SNN for MNIST \cite{cohen2017emnist}  dataset under different quantized-aware Int8, Float16 and Float32 level for PGD and BIM attacks for $\epsilon$=1. The labels $V_{th}$ refers to Threshold Voltage and $T$ refers to Time Steps for SNN models.} 
    \label{fig:mnistattack}
\end{figure*}


\begin{comment}
\begin{figure*}[!t]

\centering
	\begin{subfigure}[b]{.26\textwidth}
		\centering
		\vspace{-0.01in}
		\caption{PGD}
		{\resizebox{\textwidth}{!}{\input{Figs/cifar10/q8cifarpgd.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
	\begin{subfigure}[b]{.22\textwidth}
		\centering
		\vspace{-0.01in}
		\caption{BIM}
		{\resizebox{\textwidth}{!}{\input{Figs/cifar10/q8cifarbim.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
	\begin{subfigure}[b]{.22\textwidth}
		\centering
		\vspace{-0.01in}
		\caption{FGSM}
		{\resizebox{\textwidth}{!}{\input{Figs/cifar10/q8cifarfgsm.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
    \begin{subfigure}[b]{.22\textwidth}
		\centering
		\vspace{-0.01in}
		\caption{DF}
		{\resizebox{\textwidth}{!}{\input{Figs/cifar10/q8cifardf.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
    \label{fig:q8cifar}
\vspace{0.05in}

\centering
	\begin{subfigure}[b]{.26\textwidth}
		\centering
		\vspace{-0.01in}
		%\caption{PGD}
		{\resizebox{\textwidth}{!}{\input{Figs/cifar10/q16cifarpgd.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
	\begin{subfigure}[b]{.22\textwidth}
		\centering
		\vspace{-0.01in}
		%\caption{BIM}
		{\resizebox{\textwidth}{!}{\input{Figs/cifar10/q16cifarbim.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
	\begin{subfigure}[b]{.22\textwidth}
		\centering
		\vspace{-0.01in}
		%\caption{FGSM}
		{\resizebox{\textwidth}{!}{\input{Figs/cifar10/q16cifarfgsm.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
    \begin{subfigure}[b]{.22\textwidth}
		\centering
		\vspace{-0.01in}
		%\caption{DF}
		{\resizebox{\textwidth}{!}{\input{Figs/cifar10/q16cifardf.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
    \label{fig:q16cifar}
    \vspace{0.05in}
    \hspace{0.1in}
\centering
	\begin{subfigure}[b]{.268\textwidth}
		\centering
		\vspace{-0.1in}
		%\caption{PGD}
		{\resizebox{\textwidth}{!}{\input{Figs/cifar10/q32cifarpgd.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
	\begin{subfigure}[b]{.228\textwidth}
		\centering
        \hspace{0.2in}
		\vspace{-0.01in}
		%\caption{BIM}
		{\resizebox{\textwidth}{!}{\input{Figs/cifar10/q32cifarbim.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
	\begin{subfigure}[b]{.228\textwidth}
		\centering
        \hspace{0.05in}
		\vspace{-0.01in}
		%\caption{FGSM}
		{\resizebox{\textwidth}{!}{\input{Figs/cifar10/q32cifarfgsm.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
    \begin{subfigure}[b]{.228\textwidth}
		\centering
          \hspace{-0.25in}
		\vspace{-0.01in}
		%\caption{DF}
		{\resizebox{\textwidth}{!}{\input{Figs/cifar10/q32cifardf.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}

    \caption{Robustness of approximate and accurate SNN for CIFAR-10 dataset under different quantized-aware Int8, Float16 and Float32 (row wise) level for PGD, BIM, FGSM and DF attacks for $\epsilon$=0.9.} 
    \label{fig:cifarattack}
\end{figure*}
\end{comment}

\begin{figure}[!t]
\centering
	\begin{subfigure}[b]{.26\textwidth}
		\centering
		\vspace{-0.01in}
		\caption{MNIST}
		{\resizebox{\textwidth}{!}{\input{Figs/q32.tikz}}\label{fig:l2CR_Alx}}
	\end{subfigure}
    \caption{Accurate SNN prediction accuracy for MNIST dataset under no attack ($\epsilon$=0).} 
    \label{fig:noattack}
\end{figure}







